SOAF: Scene Occlusion-aware Neural Acoustic Field

This paper tackles the problem of novel view audio-visual synthesis along an arbitrary trajectory in an indoor scene, given the audio-video recordings from other known trajectories of the scene. Existing methods often overlook the effect of room geometry, particularly wall occlusions on sound propagation, making them less accurate in multi-room environments. In this work, we propose a new approach called Scene Occlusion-aware Acoustic Field (SOAF) for accurate sound generation. Our approach derives a global prior for the sound field using distance-aware parametric sound-propagation modeling and then transforms it based on the scene structure learned from the input video. We extract features from the local acoustic field centered at the receiver using a Fibonacci Sphere to generate binaural audio for novel views with a direction-aware attention mechanism. Extensive experiments on the real dataset RWAVS and the synthetic dataset SoundSpaces demonstrate that our method outperforms previous state-of-the-art techniques in audio generation.

==> figures/quali_result.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=1\textwidth]{figures/vis.png}
\caption{Example visual comparison of the synthesised audio (left channel) rendered from the novel view in the left image. Compared with AV-NeRF~\cite{AVNeRF}, our method attenuates more accurately the sound energy of the source audio, which is emitted from the right side of the receiver.}
\label{fig:vis}
\vspace{0.3cm}
\end{figure*}
